Gradual Domain Adaptation: Theory and Algorithms

Unsupervised domain adaptation (UDA) adapts a model from a labeled source domain to an unlabeled target domain in a one-off way. Though widely applied, UDA faces a great challenge whenever the distribution shift between the source and the target is large. Gradual domain adaptation (GDA) mitigates this limitation by using intermediate domains to gradually adapt from the source to the target domain. In this work, we first theoretically analyze gradual self-training, a popular GDA algorithm, and provide a significantly improved generalization bound compared with Kumar et al. (2020). Our theoretical analysis leads to an interesting insight: to minimize the generalization error on the target domain, the sequence of intermediate domains should be placed uniformly along the Wasserstein geodesic between the source and target domains. The insight is particularly useful under the situation where intermediate domains are missing or scarce, which is often the case in real-world applications. Based on the insight, we propose $\textbf{G}$enerative Gradual D$\textbf{O}$main $\textbf{A}$daptation with Optimal $\textbf{T}$ransport (GOAT), an algorithmic framework that can generate intermediate domains in a data-dependent way. More concretely, we first generate intermediate domains along the Wasserstein geodesic between two given consecutive domains in a feature space, then apply gradual self-training to adapt the source-trained classifier to the target along the sequence of intermediate domains. Empirically, we demonstrate that our GOAT framework can improve the performance of standard GDA when the given intermediate domains are scarce, significantly broadening the real-world application scenarios of GDA. Our code is available at https://github.com/uiuctml/GOAT.

==> sec/related_works.tex <==
\section{Related Work}\label{sec:related-works}

\paragraph{Self-Training}
Self-training, i.e., pseudo-labeling, is a popular semi-supervised learning approach~\citep{yarowsky1995unsupervised,lee2013pseudo}, which fine-tunes trained classifiers with pseudo-labels predicted on unlabelled data. There are some common techniques that can enhance self-training, e.g., adding noise to inputs or networks~\citep{xie2020self,FixMatch}, progressively assigning pseudo-labels on unlabelled data with high prediction confidence, or applying a strong regularization~\citep{arazo2020pseudo,pham2021meta}.

\paragraph{Unsupervised Domain Adaptation}
Unsupervised domain adaptation (UDA) focuses on adapting models trained on labeled data of a source domain to a target domain with unlabelled data. A number of approaches have been proposed for UDA in recent years. Invariant representation learning is one of the most popular approaches~\citep{deepCORAL,zhao2019domain}, where adversarial training is usually adopted to learn feature representations invariant between source and target domains~\citep{ajakan2014domain,ganin2016domain}. In addition, self-training (i.e., pseudo-labelling) is also adapted for UDA~\citep{liang2019distant,liang2020we,zou2018unsupervised,zou2019confidence}. In summary, pseudo-labels of unlabelled target domain data are generated by source-trained classifiers, and they are used to further fine-tune the trained classifiers. Notably, the performance of self-training degrades significantly when there is a large distribution shift between the source and target. 


\paragraph{Gradual Domain Adaptation}
Gradual domain adaptation (GDA) introduces extra intermediate domains to the existing source and target domains of UDA. In general, the intermediate domains shift from the source to the target gradually, such as rotation or time evolution~\citep{kumar2020understanding}, and GDA iteratively adapts models from the source to the target along the sequence of intermediate domains. The idea of GDA has been empirically explored in computer vision~\citep{gadermayr2018gradual,hoffman2014continuous,wulfmeier2018incremental} with various domain-specific algorithms. Recently,~\citet{kumar2020understanding} proposes a general machine learning algorithm for GDA, \textit{gradual self-training}, which outperforms vanilla self-training on several synthetic and real datasets. Moreover,~\citet{kumar2020understanding} provides a generalization error bound for gradual self-training, which is the first theoretical guarantee for GDA. In parallel,~\citet{wang2020continuously} proposes an adversarial adaptation algorithm for GDA. Later,~\citet{abnar2021gradual} proposes a variant of gradual self-training that does not need intermediate domain data, since it could generate pseudo-data for intermediate domains. In GDA, the intermediate domains are given (i.e., ordering domains based on their distance to the source/target domain),~\citet{chen2021gradual} removes the requirement of the domain order by proposing a method called Intermediate Domain Labeler (IDOL).~\citet{chen2021gradual} shows gradual self-training with IDOL could obtain good performance even without the domain order. Recently,~\citet{zhou2022online} proposed an algorithm under the teacher-student paradigm with active query strategy to tackle the gradual adaptation problem.~\citet{dong2022algorithms} studied a slightly different setting where labeled data is also available during the intermediate domains. In addition, one may notice that GDA has a setting similar to temporal domain generalization~\citep{koh2021wilds,ye2022future}, while the latter has available labels in intermediate domains instead.

==> tables/OT_ablation.tex <==
\begin{table}[t!]
\small
\centering
\caption{Ablation study on the transport plan used in GOAT (i.e., Algo. \ref{algo:main})}\label{tab:ablation}
    \begin{tabular}{lcccc} 
    \toprule 
    & \multicolumn{3}{c}{\# Generated Domains}\\
                      & 1  & 2 & 3  \\
    \midrule
    GOAT with \textbf{Random} Transport Plan   & 55.32 $\pm$ 3.14 & 62.52 $\pm$ 2.61 & 62.04 $\pm$ 1.35\\
    GOAT with \textbf{Uniform} Transport Plan &  57.26 $\pm$ 3.55 & 62.44 $\pm$ 2.78 &  62.40 $\pm$ 1.40 \\
    GOAT with \textbf{Optimal Transport (OT)} Plan & \textbf{67.97 $\pm$ 1.37} & \textbf{66.97 $\pm$ 2.24} & \textbf{69.12 $\pm$ 2.18} \\
    \midrule
    GOAT with \textbf{Ground-Truth} Transport Plan & 67.90 $\pm$ 3.65 & 69.47 $\pm$ 1.93 & 71.36 $\pm$ 1.92\\
    \bottomrule
    \end{tabular}
\end{table}

==> tables/mnist.tex <==
\begin{table}[t!]
\small
\caption{Accuracy (\%) on Rotated MNIST.}
\begin{tabular}{c|cccc|c}
\toprule

\diagbox{\# Oracle}{\# Generated} & 1                             & 2                             & 3       &4                      & GST                                 \\
\midrule
0                    & 48.49 $\pm$ 2.24 &47.17 $\pm$ 1.70 & 48.17 $\pm$ 2.70 & 47.47 $\pm$2.84 & \textbf{50.27 $\pm$ 0.68}       \\
1                    & 55.15 $\pm$ 2.55 & 54.60 $\pm$ 1.63 & \textbf{57.08 $\pm$ 2.21} & 56.19$\pm$1.93 & 56.31 $\pm$ 1.93       \\
2                    & 67.97 $\pm$ 1.37 & 66.97 $\pm$ 2.24 & 69.12 $\pm$ 2.18 & \textbf{70.31$\pm$2.42} &61.58  $\pm$ 2.10      \\
3                    & 73.93 $\pm$ 1.06 & \textbf{74.35 $\pm$ 1.79} & 73.21 $\pm$ 2.02 & 74.00$\pm$2.31 & 66.30  $\pm$ 2.04      \\
4                    & 83.77 $\pm$ 1.95 & 84.01 $\pm$ 1.64 & \textbf{86.41 $\pm$ 1.96} & 82.69$\pm$1.82 &75.48 $\pm$ 2.00       \\   
\bottomrule    
\label{Tab:mnist}        
\end{tabular}
\end{table}

==> tables/portraits.tex <==
\begin{table}[t!]
\small
\caption{Accuracy (\%) on Portraits.}
\begin{tabular}{c|cccc|c}
\toprule
\diagbox{\# Oracle}{\# Generated} & 1                             & 2                             & 3                  & 4           & GST                                 \\
\midrule
0                    & 73.99 $\pm$ 1.25 & 73.51 $\pm$ 2.15 & 73.57 $\pm$ 2.45 & \textbf{74.24 $\pm$2.45} & 73.25 $\pm$ 1.30       \\
1                    & 76.41 $\pm$ 1.31 & 75.54 $\pm$ 2.55 & \textbf{76.75 $\pm$ 1.50} & 74.68$\pm$1.72 & 74.53 $\pm$ 1.56       \\
2                    & 77.39 $\pm$ 2.09 & 79.39 $\pm$ 2.39 & \textbf{79.85 $\pm$ 1.16} & 77.23$\pm$0.90 & 77.02  $\pm$ 1.30      \\
3                    & 80.89 $\pm$ 1.63 & 81.82 $\pm$ 1.32 & \textbf{82.27 $\pm$ 1.28} & 81.31$\pm$1.48 & 80.65  $\pm$ 2.30      \\
4                    & 82.75 $\pm$ 1.47 & \textbf{83.57 $\pm$ 1.47} & 82.41 $\pm$ 1.36 & 81.76$\pm$1.59 & 81.95 $\pm$ 1.38       \\   
\bottomrule     
\label{Tab:portraits}           
\end{tabular}
\end{table}

==> tables/small_covi.tex <==
\begin{table}
\centering
\captionof{table}{\small Comparison with CoVi \cite{na2022covi} on Portraits.}
\vspace{-0.5em}
{\small
\setlength\tabcolsep{0.4em}
\begin{tabular}{c cc c}
\toprule
{\# Given Domains} & GST & CoVi & GOAT   \\
\midrule
0 & 73.3$\pm$1.3 & 73.7$\pm$3.5 & \textbf{74.2$\pm$2.5}     \\
1 & 74.5$\pm$1.6 & 75.3$\pm$1.8 & \textbf{76.8$\pm$1.5} \\
2 & 77.0$\pm$1.3 & \textbf{79.8$\pm$3.0} & \textbf{79.9$\pm$1.2}  \\
3 & 80.7$\pm$2.3 & \textbf{82.3$\pm$1.4} & \textbf{82.3$\pm$1.3} \\
4  & 82.0$\pm$1.4 & 83.1$\pm$1.9 & \textbf{83.6$\pm$1.5}\\   
\bottomrule     
\label{Tab:covi}           
\end{tabular}
}
\end{table}
